Endo-Depth-and-Motion: Reconstruction and Tracking in Endoscopic Videos using Depth Networks and Photometric Constraints

Estimating a scene reconstruction and the camera motion from in-body videos is challenging due to several factors, e.g. the deformation of in-body cavities or the lack of texture. In this paper we present Endo-Depth-and-Motion, a pipeline that estimates the 6-degrees-of-freedom camera pose and dense 3D scene models from monocular endoscopic videos. Our approach leverages recent advances in self-supervised depth networks to generate pseudo-RGBD frames, then tracks the camera pose using photometric residuals and fuses the registered depth maps in a volumetric representation. We present an extensive experimental evaluation in the public dataset Hamlyn, showing high-quality results and comparisons against relevant baselines. We also release all models and code for future comparisons.

==> Sections/backuptablereducida.tex <==
\begin{table*}[]
    \normalsize
    \centering
    \resizebox{\textwidth}{!} {%
    \begin{tabular}{ c | c  c  c  c  c  c  c  c  c  c  c  c  c  c  c  c  c  c  c  c  c | c  }
    
        \hline
        \cellcolor{Orange}Abs Rel & 1 & 4 & 5 & 6 & 8 & 11 & 12 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & mean \\ \hline
        MONOCULAR LOSS  &   0.260  &   0.059  &   0.064  &   0.152  &   0.132  &   0.112  &   0.089  &   0.162  &   0.109  &   0.100  &   0.232  &   0.308  &   0.296  &   0.115  &   0.123  &   0.230  &   0.252  &   0.241  &   0.146  &   0.157  &   0.178   &   0.167 \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        STEREO LOSS    &   \textbf{0.091}  &   \textbf{0.038}  &   \textbf{0.047}  &   \textbf{0.080}  &   0.120  &   0.092  &   \textbf{0.040}  &   \textbf{0.136}  &   \textbf{0.070}  &   \textbf{0.072}  &   \textbf{0.195}  &   \textbf{0.230}  &   \textbf{0.184}  &   0.109  &   \textbf{0.108}  &   \textbf{0.158}  &   \textbf{0.166}  &   \textbf{0.183}  &   \textbf{0.141}  &   \textbf{0.131}  &   \textbf{0.128}  &   0.120  \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        MON+STER LOSS   &   0.193  &   0.040  &   0.073  &   0.432  &   \textbf{0.114}  &   \textbf{0.079}  &   0.109  &   0.163  &   0.088  &   0.095  &   0.222  &   \textbf{0.232}  &   0.272  &   \textbf{0.095}  &   0.137  &   0.211  &   0.215  &   0.201  &   0.171  &   0.168  &   0.152   &   0.165 \\ 
        \hline
        
        \hline
        \cellcolor{Orange}Sq Rel & 1 & 4 & 5 & 6 & 8 & 11 & 12 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & mean \\ \hline
        MONOCULAR LOSS  &  19.775  &   0.269  &   0.335  &   6.461  &   2.738  &   1.491  &   1.629  &   3.859  &   0.796  &   1.102  &   6.175  &  10.802  &  12.437  &   1.093  &   1.681  &   5.689  &   9.159  &   6.260  &   \textbf{2.318}  &   2.874  &   4.247   &   4.819 \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        STEREO LOSS    &   \textbf{1.429}  &   \textbf{0.160}  &   \textbf{0.186}  &   \textbf{1.057}  &   1.951  &   1.332  &   \textbf{0.651}  &   \textbf{2.855}  &   \textbf{0.425}  &   \textbf{0.751}  &   \textbf{5.344}  &   6.994  &   \textbf{4.379}  &   1.084  &   \textbf{1.581}  &   \textbf{3.147}  &   \textbf{4.954}  &   \textbf{3.664}  &   2.471  &   \textbf{2.407}  &   \textbf{2.371}   &   2.343 \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        MON+STER LOSS   &   9.251  &   0.193  &   0.458  &  56.218  &   \textbf{1.906}  &   \textbf{0.931}  &   1.442  &   3.861  &   0.643  &   1.111  &   5.676  &   \textbf{6.415}  &   9.699  &   \textbf{0.723}  &   2.344  &   4.772  &   7.936  &   4.136  &   3.224  &   3.072  &   3.204   &   6.058 \\
        \hline
    
        \hline
        \cellcolor{Orange}RMSE & 1 & 4 & 5 & 6 & 8 & 11 & 12 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & \%-best \\ \hline
        MONOCULAR LOSS  &  30.617  &   3.405  &   3.859  &  23.488  &  14.301  &   9.978  &  10.232  &  14.142  &   5.279  &   6.796  &  19.540  &  28.302  &  24.495  &   7.057  &   9.272  &  18.805  &  21.619  &  18.321  &  \textbf{10.754}  &  12.872  &  15.517    &   4.8 \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        STEREO LOSS   &   \textbf{9.792}  &   \textbf{2.385}  &   \textbf{2.855}  &  \textbf{10.653}  &  \textbf{11.296}  &   9.156  &   \textbf{6.156}  &  \textbf{11.833}  &   \textbf{3.537}  &   \textbf{5.258 } &  \textbf{17.793}  &  \textbf{21.772}  &  \textbf{15.723}  &   6.816  &   \textbf{8.760}  &  \textbf{13.848}  &  \textbf{16.003}  &  \textbf{14.522}  &  11.022  &  \textbf{11.862}  &  \textbf{11.072}   &   \textbf{85.7} \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        MON+STER LOSS   &  21.042  &   2.572  &   4.472  &  55.892  &  11.729  &  \textbf{ 7.790 } &  10.160  &  13.068  &   4.798  &   6.648  &  18.868  &  21.984  &  22.274  &   \textbf{5.735}  &  10.657  &  17.145  &  19.263  &  15.523  &  12.489  &  13.506  &  12.570   &   9.5 \\ 
        \hline
        
        \hline
        \cellcolor{Orange}RMSE log & 1 & 4 & 5 & 6 & 8 & 11 & 12 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & \%-best \\ \hline
        MONOCULAR LOSS  &   0.287  &   0.075  &   0.083  &   0.187  &   0.188  &   0.159  &   0.126  &   0.217  &   0.156  &   0.130  &   0.272  &   0.361  &   0.320  &   0.145  &   0.152  &   0.271  &   0.284  &   0.294  &   0.186  &   0.197  &   0.213   &   0.205 \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        STEREO LOSS   &   \textbf{0.114}  &   \textbf{0.052}  &   \textbf{0.061}  &   \textbf{0.099}  &   \textbf{0.154}  &   0.126  &   \textbf{0.070}  &   \textbf{0.183}  &   \textbf{0.099}  &   \textbf{0.099}  &   \textbf{0.239}  &   \textbf{0.279}  &   \textbf{0.230}  &   0.138  &   \textbf{0.141}  &   \textbf{0.199}  &   \textbf{0.206}  &   \textbf{0.226}  &   \textbf{0.179}  &   \textbf{0.169}  &   \textbf{0.161}   &   0.154 \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        MON+STER LOSS   &   0.230  &   \textbf{0.056}  &   0.093  &   0.400  &   \textbf{0.153}  &   \textbf{0.112}  &   0.146  &   0.212  &   0.144  &   0.123  &   0.262  &   \textbf{0.278}  &   0.310  &   \textbf{0.118}  &   0.173  &   0.251  &   0.254  &   0.245  &   0.213  &   0.208  &   0.185   &   0.198\\
        \hline
        
        
        \hline
        \cellcolor{SpringGreen}\delta < 1.25^1 & 1 & 4 & 5 & 6 & 8 & 11 & 12 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & \%-best \\ \hline
        MONOCULAR LOSS  &   0.747  &   \textbf{0.989}  &   \textbf{0.995}  &   0.810  &   0.810  &   0.864  &   0.921  &   0.767  &   0.887  &   0.915  &   0.586  &   0.453  &   0.557  &   0.865  &   0.860  &   0.567  &   0.647  &   0.595  &   0.804  &   0.776  &   0.735   &   0.769 \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        STEREO LOSS   &   \textbf{0.928}  &   \textbf{0.989}  &   \textbf{0.999}  &   \textbf{0.952}  &   \textbf{0.866}  &   0.941  &   \textbf{0.984}  &   \textbf{0.808}  &   \textbf{0.952}  &   \textbf{0.948}  &   \textbf{0.717}  &   \textbf{0.628}  &   \textbf{0.727}  &   0.876  &   \textbf{0.885}  &   \textbf{0.761}  &   \textbf{0.810}  &   \textbf{0.711}  &   \textbf{0.832}  &   \textbf{0.837}  &   \textbf{0.842}   &   0.857 \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        MON+STER LOSS   &   0.780  &   \textbf{0.987}  &   0.968  &   0.610  &   0.857  &   \textbf{0.962}  &   0.888  &   0.776  &   0.908  &   0.917  &   0.630  &   0.574  &   0.583  &   \textbf{0.930}  &   0.838  &   0.619  &   0.754  &   0.642  &   0.768  &   0.738  &   0.791   &   0.787 \\
        \hline
        
        \hline
        \cellcolor{SpringGreen}\delta < 1.25^2 & 1 & 4 & 5 & 6 & 8 & 11 & 12 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & \%-best \\ \hline
        MONOCULAR LOSS  &   0.890  &   \textbf{1.000}  &   \textbf{1.000}  &   0.963  &   0.955  &   0.989  &   0.984  &   0.924  &   0.975  &   0.988  &   0.884  &   0.764  &   0.823  &   0.993  &   \textbf{0.985}  &   0.891  &   0.856  &   0.872  &   \textbf{0.962}  &   0.956  &   0.942   &   0.933 \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        STEREO LOSS   &   \textbf{0.989}  &   0.999  &   \textbf{1.000}  &   \textbf{0.999}  &   \textbf{0.980}  &   0.989  &   0.991  &   \textbf{0.950}  &   \textbf{0.992}  &   \textbf{0.990}  &   \textbf{0.915}  &   0.870  &   \textbf{0.921}  &   0.990  &   0.980  &   \textbf{0.955}  &   \textbf{0.923}  &   \textbf{0.930}  &   0.960  &   \textbf{0.967}  &   \textbf{0.972}   &   0.965 \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        MON+STER LOSS   &   0.946  &   0.999  &   0.999  &   0.861  &   \textbf{0.980}  &   \textbf{0.993}  &   \textbf{0.993}  &   0.936  &   0.971  &   0.985  &   0.893  &   \textbf{0.873}  &   0.842  &   \textbf{0.999}  &   0.962  &   0.910  &   0.881  &   0.922  &   0.944  &   0.952  &   0.959   &   0.943 \\ 
        \hline
        
        \hline
        \cellcolor{SpringGreen}\delta < 1.25^3 & 1 & 4 & 5 & 6 & 8 & 11 & 12 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & \%-best \\ \hline
        MONOCULAR LOSS  &   0.940  &   \textbf{1.000}  &   \textbf{1.000}  &   0.989  &   0.989  &   0.994  &   0.995  &   0.978  &   0.995  &   0.997  &   0.980  &   0.937  &   0.941  &   \textbf{1.000}  &   \textbf{0.998}  &   0.986  &   0.940  &   0.959  &   \textbf{0.995}  &   0.993  &   0.990   &   0.981 \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        STEREO LOSS   &   \textbf{0.998}  &   \textbf{1.000}  &   \textbf{1.000}  &   \textbf{1.000}  &   0.996  &   0.995  &   0.995  &   \textbf{0.986}  &   \textbf{0.999}  &   0.998  &   0.977  &   0.967  &   \textbf{0.978}  &   0.999  &   \textbf{0.998}  &   \textbf{0.991}  &   \textbf{0.975}  &   \textbf{0.992}  &   0.993  &   \textbf{0.994}  &   \textbf{0.995}   &   0.992 \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        MON+STER LOSS   &   0.974  &   \textbf{1.000}  &   \textbf{1.000}  &   0.898  &   \textbf{0.997}  &   \textbf{0.996}  &   \textbf{0.996}  &   0.977  &   0.993  &   \textbf{0.999}  &   \textbf{0.985}  &   \textbf{0.983}  &   0.948  &   \textbf{1.000}  &   0.996  &   0.990  &   0.945  &   0.989  &   0.985  &   \textbf{0.994}  &   0.991   &   0.983 \\
        \hline
        
        
    \end{tabular}%
    }
    \caption{Evaluation of Endo-Depth for the Hamlyn sequences with Local Scale.}
    \label{tab:endodepth_eval_red}
\end{table*}


\begin{table*}[]
    \centering
    \resizebox{\textwidth}{!} {%
    \begin{tabular}{| c || c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | }

    \multicolumn{23}{c}{} \\
    \multicolumn{23}{l}{\large Trained with stereo losses, evaluated with global scale} \\
        \hline
        test video & 1 & 4 & 5 & 6 & 8 & 11 & 12 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & mean \\ \hline
        \cellcolor{Orange}Abs Rel    &   0.573  &   0.070  &   0.062  &   0.342  &   0.642  &   0.168  &   0.203  &   0.209  &   0.105  &   0.174  &   0.222  &   0.255  &   0.236  &   0.192  &   0.128  &   0.198  &   0.182  &   0.365  &   0.158  &   0.156  &   0.224  &  0.232   \\ \arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{Orange}Sq Rel    &  29.813  &   0.337  &   0.262  &  19.045  &  32.455  &   2.724  &   3.323  &   3.916  &   0.576  &   2.375  &   8.182  &   8.428  &   6.662  &   3.429  &   1.713  &   5.538  &   5.478  &  13.119  &   2.932  &   2.919  &   5.067  &  7.538   \\ \arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{Orange}RMSE    &  44.538  &   3.605  &   3.570  &  29.569  &  38.724  &  12.649  &  15.521  &  13.724  &   4.152  &   9.971  &  20.678  &  24.102  &  18.435  &  11.130  &   9.605  &  16.963  &  16.622  &  24.723  &  11.799  &  13.138  &  17.851  &  17.194   \\ \arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{Orange}RMSE log    &   0.452  &   0.081  &   0.075  &   0.273  &   0.484  &   0.183  &   0.245  &   0.232  &   0.130  &   0.181  &   0.269  &   0.304  &   0.271  &   0.200  &   0.155  &   0.233  &   0.216  &   0.352  &   0.195  &   0.195  &   0.294  &  0.239 \\ \arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{SpringGreen}\delta < 1.25    &   0.158  &   0.990  &   0.999  &   0.632  &   0.199  &   0.800  &   0.488  &   0.696  &   0.941  &   0.837  &   0.763  &   0.555  &   0.663  &   0.718  &   0.852  &   0.733  &   0.815  &   0.524  &   0.772  &   0.774  &   0.467  &  0.684 \\ \arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{SpringGreen}\delta < 1.25^2    &   0.492  &   1.000  &   1.000  &   0.787  &   0.545  &   0.983  &   0.983  &   0.935  &   0.988  &   0.972  &   0.867  &   0.840  &   0.867  &   0.940  &   0.989  &   0.902  &   0.917  &   0.769  &   0.956  &   0.960  &   0.828  &  0.882 \\ \arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{SpringGreen}\delta < 1.25^3    &   0.894  &   1.000  &   1.000  &   0.886  &   0.792  &   0.994  &   0.990  &   0.980  &   0.997  &   0.996  &   0.943  &   0.961  &   0.961  &   0.996  &   0.998  &   0.975  &   0.969  &   0.908  &   0.990  &   0.993  &   0.975  &  0.962 \\ \hline
        
    \multicolumn{23}{c}{} \\
    \multicolumn{23}{l}{\large Trained with monocular + stereo losses, evaluated with global scale} \\
        \hline
        test video & 1 & 4 & 5 & 6 & 8 & 11 & 12 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & mean \\ \hline
        \cellcolor{Orange}Abs Rel    &   0.312  &   0.070  &   0.079  &   0.571  &   0.754  &   0.086  &   0.295  &   0.514  &   0.719  &   0.396  &   0.343  &   0.262  &   0.379  &   0.279  &   0.208  &   0.267  &   0.273  &   0.447  &   0.420  &   0.347  &   0.189  &  0.343\\ \arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{Orange}Sq Rel    &  18.939  &   0.392  &   0.530  &  83.030  &  41.415  &   1.057  &   6.415  &  13.947  &  15.758  &   9.142  &  12.983  &   7.743  &  12.800  &   4.599  &   4.640  &   8.038  &   7.842  &  17.415  &  13.131  &   9.939  &   3.928  &  13.985\\ \arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{Orange}RMSE    &  27.863  &   3.690  &   4.799  &  65.822  &  44.831  &   8.237  &  20.921  &  23.659  &  20.948  &  19.805  &  26.075  &  24.948  &  30.643  &  13.813  &  14.505  &  20.749  &  21.462  &  28.698  &  24.522  &  22.421  &  15.660  &  23.051 \\ \arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{Orange}RMSE log    &   0.306  &   0.083  &   0.100  &   0.472  &   0.547  &   0.120  &   0.388  &   0.431  &   0.546  &   0.347  &   0.353  &   0.311  &   0.550  &   0.263  &   0.226  &   0.292  &   0.289  &   0.407  &   0.385  &   0.334  &   0.242  &  0.333 \\ \arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{SpringGreen}\delta < 1.25    &   0.606  &   0.984  &   0.961  &   0.455  &   0.153  &   0.956  &   0.160  &   0.299  &   0.071  &   0.276  &   0.569  &   0.486  &   0.182  &   0.470  &   0.700  &   0.613  &   0.529  &   0.413  &   0.401  &   0.438  &   0.609  &  0.492 \\ \arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{SpringGreen}\delta < 1.25^2    &   0.838  &   1.000  &   0.999  &   0.765  &   0.381  &   0.992  &   0.752  &   0.595  &   0.220  &   0.810  &   0.794  &   0.822  &   0.425  &   0.938  &   0.927  &   0.839  &   0.889  &   0.698  &   0.671  &   0.802  &   0.911  &  0.765 \\ \arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{SpringGreen}\delta < 1.25^3    &   0.958  &   1.000  &   1.000  &   0.872  &   0.724  &   0.995  &   0.971  &   0.830  &   0.853  &   0.973  &   0.893  &   0.982  &   0.742  &   0.998  &   0.983  &   0.962  &   0.958  &   0.874  &   0.926  &   0.956  &   0.993  &  0.926 \\ \hline
    \end{tabular}%
    }
    \caption{Evaluation of Endo-Depth for the Hamlyn sequences.}
    \label{tab:endodepth_eval_global_scale}
\end{table*}



% Endodepth vs IsoNRSfM
% Mono - stereo - mono+stereo - IsoNRSfM of SD-DefSLAM
\begin{table*}[]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{c || c | c | c | c || c | c | c | c || c | c | c | c || c | c | c | c |}
    \cline{2-17}
                                                                  & \multicolumn{4}{c||}{IsoNRSfM - Local scale}&\multicolumn{4}{c||}{Endo-Depth (stereo loss)}                & \multicolumn{4}{c||}{Endo-Depth (mono loss)} & \multicolumn{4}{c|}{Endo-Depth (monocular + stereo loss)} \\ \hline
    \multicolumn{1}{|c||}{test video}                             & 1           & 4          & 19          & 20          & 1      & 4     & 19     & 20     & 1           & 4          & 19          & 20          & 1      & 4     & 19     & 20          \\ \hline
    \multicolumn{1}{|c||}{\cellcolor{Orange}Abs Rel}              &\underline{0.097}        &      0.048 & {\bf 0.062} &{\bf 0.064}  &{\bf0.083}&\underline{0.024}&\underline{0.169}   &0.120     &0.293        & 0.054      & 0.235       & 0.134       & 0.213  &{\bf0.023}&0.284& \underline{0.087}    \\ \hline
    \multicolumn{1}{|c||}{\cellcolor{Orange}Sq Rel}               &\underline{2.563}        & 0.185      & {\bf 0.769} &{\bf 0.578}  &{\bf1.379}&{\bf0.051}&\underline{5.275}&1.212  & 26.497      & 0.204      & 7.432       & 1.487       & 11.822 & \underline{0.052} & 11.768 & \underline{0.603}    \\ \hline
    \multicolumn{1}{|c||}{\cellcolor{Orange}RMSE}                 &\underline{19.815}       &2.698       &{\bf 6.478}  & \underline{6.420}       &{\bf9.361}&\underline{1.432}&\underline{16.213}  &7.491  &34.382       & 2.937      & 18.640      & 8.354       & 23.553 &{\bf1.428}  &  24.026&{\bf5.401}\\ \hline
    \multicolumn{1}{|c||}{\cellcolor{Orange}RMSE log}             &{\bf 0.015}  &{\bf 0.004} &{\bf 0.009}  &{\bf 0.007}  & \underline{0.109}  & \underline{0.032} & \underline{0.228}  & 0.147  & 0.310       & 0.068      & 0.264       & 0.168       & 0.251  & 0.032 & 0.328  & \underline{0.108}   \\ \hline
    \multicolumn{1}{|c||}{\cellcolor{SpringGreen}\delta < 1.25}   &{\bf 0.930}  &   0.997    &{\bf 0.960}  &{\bf 0.988}  & \underline{0.926}  &{\bf1.000}&\underline{0.796}& 0.845  & 0.741       & 0.997      & 0.595       & 0.799       & 0.762  &{\bf1.000}&0.689& \underline{0.959}  \\ \hline
    \multicolumn{1}{|c||}{\cellcolor{SpringGreen}\delta < 1.25^2} &{\bf 0.998}  &{\bf1.000}  &{\bf 0.997}  &{\bf 1.000}  & \underline{0.988}  &{\bf1.000}& 0.910  & 0.995  & 0.881       & {\bf1.000} & \underline{0.921}       & 0.988       & 0.931  &{\bf1.000} & 0.832  & \underline{0.999} \\ \hline
    \multicolumn{1}{|c||}{\cellcolor{SpringGreen}\delta < 1.25^3} &{\bf 0.999}  &{\bf1.000}  &{\bf 1.000}  &{\bf1.000}   & \underline{0.998}  &{\bf1.000}& 0.964  &{\bf1.000}  & 0.928       & {\bf1.000} & 0.988       & \underline{0.999}       & 0.965  &{\bf1.000} & 0.909  &{\bf1.000}  \\ \hline
    \end{tabular}%
    }
    \caption{IsoNRSfM (taken from~\cite{rodriguez2020sd}) vs. Endo-Depth (trained with monocular, stereo and monocular + stereo losses). All methods use local scale of Eq. \ref{eq:local_factor_2}. $RMSE$ in mm, $RMSE_{log}$ in log mm. Best results are boldfaced, second ones underlined.}
    \label{tab:endodepth_vs_isonrsfm}
\end{table*}

==> Sections/bacuptablecomparison.tex <==
\begin{table}[t!]
    \small
    \centering
    \resizebox{\linewidth}{!} {%
    \begin{tabular}{ c  c  c  c  c  c  }
        \multicolumn{2}{c}{} & \multicolumn{4}{c}{\textbf{Sequence}} \\
        \noalign{\vskip 1mm} 
        \cline{3-6}
        \noalign{\vskip 1mm}   
        \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{Method}} & 1 & 4 & 19 & 20 \\
        \noalign{\vskip 1mm} 
        \hline
        \noalign{\vskip 1mm}  
        
        \cellcolor{Dandelion} & IsoNRSfM \cite{parashar2017IsoNRSfM} &\underline{0.097}        &      0.048 & {\bf 0.062} &{\bf 0.064} \\
        \cellcolor{Dandelion} & \textbf{ours} Mono  &  0.293        & 0.054      & 0.235       & 0.134   \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{Dandelion} & \textbf{ours} Stereo   &   {\bf0.083}&\underline{0.024}&\underline{0.169}   &0.120  \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{Dandelion} \multirow{-4}{*}{Abs Rel}& \textbf{ours} Mono + Stereo   &   0.213  &{\bf0.023}&0.284& \underline{0.087}\\ 
        %\hline
        \noalign{\vskip 1mm} 
        \hline
        \noalign{\vskip 1mm}   
        
        \cellcolor{Dandelion} & IsoNRSfM \cite{parashar2017IsoNRSfM} &\underline{2.563}        & 0.185      & {\bf 0.769} &{\bf 0.578}\\
        \cellcolor{Dandelion} & \textbf{ours} Mono  &  26.497      & 0.204      & 7.432       & 1.487   \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{Dandelion} & \textbf{ours} Stereo   &   {\bf1.379}&{\bf0.051}&\underline{5.275}&1.212  \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{Dandelion} \multirow{-4}{*}{Sq Rel}& \textbf{ours} Mono + Stereo   &   11.822 & \underline{0.052} & 11.768 & \underline{0.603} \\ 
        %\hline
        \noalign{\vskip 1mm} 
        \hline
        \noalign{\vskip 1mm} 
        
        \cellcolor{Dandelion} & IsoNRSfM \cite{parashar2017IsoNRSfM} &\underline{19.815}       &2.698       &{\bf 6.478}  & \underline{6.420}\\
        \cellcolor{Dandelion} & \textbf{ours} Mono  &  34.382       & 2.937      & 18.640      & 8.354  \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{Dandelion} & \textbf{ours} Stereo   &   {\bf9.361}&\underline{1.432}&\underline{16.213}  &7.491  \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{Dandelion} \multirow{-4}{*}{RMSE}& \textbf{ours} Mono + Stereo   &   23.553 &{\bf1.428}  &  24.026&{\bf5.401} \\ 
        %\hline
        \noalign{\vskip 1mm} 
        \hline
        \noalign{\vskip 1mm} 
        
        \cellcolor{Dandelion} & IsoNRSfM \cite{parashar2017IsoNRSfM} &{\bf 0.015}  &{\bf 0.004} &{\bf 0.009}  &{\bf 0.007}\\
        \cellcolor{Dandelion} & \textbf{ours} Mono  &  0.310       & 0.068      & 0.264       & 0.168   \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{Dandelion} & \textbf{ours} Stereo   &   \underline{0.109}  & \underline{0.032} & \underline{0.228}  & 0.147 \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{Dandelion} \multirow{-4}{*}{RMSE\textsubscript{log}}& \textbf{ours} Mono + Stereo   &   0.251  & 0.032 & 0.328  & \underline{0.108} \\ 
        %\hline
        \noalign{\vskip 1mm} 
        \hline
        \noalign{\vskip 1mm} 
        
        \cellcolor{Orchid} & IsoNRSfM \cite{parashar2017IsoNRSfM} &{\bf 0.930}  &   0.997    &{\bf 0.960}  &{\bf 0.988}\\
        \cellcolor{Orchid} & \textbf{ours} Mono  & 0.741       & 0.997      & 0.595       & 0.799   \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{Orchid} & \textbf{ours} Stereo   &   \underline{0.926}  &{\bf1.000}&\underline{0.796}& 0.845 \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{Orchid} \multirow{-4}{*}{$\delta < 1.25^{1}$}& \textbf{ours} Mono + Stereo   &   0.762  &{\bf1.000}&0.689& \underline{0.959}\\ 
        %\hline
        \noalign{\vskip 1mm} 
        \hline
        \noalign{\vskip 1mm} 
        
        \cellcolor{Orchid} & IsoNRSfM \cite{parashar2017IsoNRSfM} &{\bf 0.998}  &{\bf1.000}  &{\bf 0.997}  &{\bf 1.000}\\
        \cellcolor{Orchid} & \textbf{ours} Mono  & 0.881       & {\bf1.000} & \underline{0.921}       & 0.988   \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{Orchid} & \textbf{ours} Stereo   &   \underline{0.988}  &{\bf1.000}& 0.910  & 0.995 \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{Orchid} \multirow{-4}{*}{$\delta < 1.25^2$}& \textbf{ours} Mono + Stereo   &   0.931  &{\bf1.000} & 0.832  & \underline{0.999}\\ 
        %\hline
        \noalign{\vskip 1mm} 
        \hline
        \noalign{\vskip 1mm} 
        
        \cellcolor{Orchid} & IsoNRSfM \cite{parashar2017IsoNRSfM} &{\bf 0.999}  &{\bf1.000}  &{\bf 1.000}  &{\bf1.000}\\
        \cellcolor{Orchid} & \textbf{ours} Mono  & 0.928       & {\bf1.000} & \underline{0.988}       & 0.999 \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{Orchid} & \textbf{ours} Stereo   &   \underline{0.998}  &{\bf1.000}& 0.964  &{\bf1.000} \\ %\arrayrulecolor{gray}\hline\arrayrulecolor{black}
        \cellcolor{Orchid} \multirow{-4}{*}{$\delta < 1.25^3$}& \textbf{ours} Mono + Stereo   &  0.965  &{\bf1.000} & 0.909  &{\bf1.000} \\ 
        %\hline
        \noalign{\vskip 1mm} 
        \hline
        \noalign{\vskip 1mm} 
        
    \end{tabular}%
    }
    \caption{\emph{Endo-Depth} vs. {IsoNRSfM}\cite{parashar2017IsoNRSfM} in {Hamlyn} sequences.  $\text{Abs}_{\text{rel}}$ and RMSE in [mm], $\text{RMSE}_{\text{log}}$ in [log mm]. }
    \vspace{-1mm}
    \label{tab:endodepth_eval_red}
\end{table}
